PRIMA: Planner-Reasoner Inside a Multi-task Reasoning Agent

We consider the problem of multi-task reasoning (MTR), where an agent can solve multiple tasks via (first-order) logic reasoning. This capability is essential for human-like intelligence due to its strong generalizability and simplicity for handling multiple tasks. However, a major challenge in developing effective MTR is the intrinsic conflict between reasoning capability and efficiency. An MTR-capable agent must master a large set of "skills" to tackle diverse tasks, but executing a particular task at the inference stage requires only a small subset of immediately relevant skills. How can we maintain broad reasoning capability and also efficient specific-task performance? To address this problem, we propose a Planner-Reasoner framework capable of state-of-the-art MTR capability and high efficiency. The Reasoner models shareable (first-order) logic deduction rules, from which the Planner selects a subset to compose into efficient reasoning paths. The entire model is trained in an end-to-end manner using deep reinforcement learning, and experimental studies over a variety of domains validate its effectiveness.

==> exp.tex <==
\section{Experiments and Results}
\label{sec:exp}
The experiments are conducted to investigate the following questions empirically. i) How do VOMPS\&ACE-STORM compare with state-of-art off-policy policy gradient methods, such as GeoffPAC~\citep{geoffpac}, ACE, DDPG~\citep{lillicrap2015continuous}, and TD3~\citep{fujimoto2018addressing}?  ii) How do VOMPS\&ACE-STORM compare with on-policy variance-reduced policy gradient methods, e.g., SVRPG~\citep{svrpg} and SRVR-PG~\citep{sarahpg}? iii) How is VOMPS\&ACE-STORM resilient to action noise in policy gradient methods?

Since the tasks for original domains are episodic, e.g., \texttt{CartPoleContinuous-v0}, \texttt{Hopper-v2} and \texttt{HalfCheetah-v2}, we modify them as continuing tasks following ~\citep{geoffpac}--- the discount factor $\gamma$ is set to $0.99$ for all non-terminal states and $0$ for terminal states. The environment is reset to the initial state if the agent reaches the terminal state.
Therefore, simulation-based cumulative rewards (Monte Carlo return) by executing the (learned) policy $\pi$ is used as the performance metric, while results of episodic return are also provided in the Appendix.
All the curves in the results are averaged over $10$ runs, where the solid curve indicates the mean and the shaded regions around the mean curve indicate standard deviation errors. To better visualize the plots, curves are smoothed by a window of size
$20$. Shorthands ``1K'' represents $10^3$, and ``1M'' represents $10^6$. 
In the off-policy setting, the behavior policy $\mu$ follows a fixed uniform distribution. VOMPS, ACE-STORM, GeoffPAC, and ACE have the same critic component in all experiments for a fair comparison.
%


\subsection{Tabular off-policy policy gradient}
%
We first compare the performance of ACE, GeoffPAC, ACE-STORM, and VOMPS on the two-circle MDP domain~\citep{imani2018off,geoffpac} in terms of their dynamic and asymptotic solutions. In the two-circle MDP, there are a finite number of states, and an agent only decides at state \texttt{A} on either transitioning to state \texttt{B} or state \texttt{C}, whereas the transitions at other states will always be deterministic. The discount factor $\gamma = 0.6$ and rewards are $0$ unless specified on the edge as shown in Fig.~\ref{fig:circle}.
%
\begin{figure*}[htb!]
\begin{subfigure}{.5\textwidth}
  \centering
%   \includegraphics[height=3.5cm,width=4cm]{figures/two-circle.png}
    \includegraphics[height=2.5cm,width=.6\textwidth]{figures/two-circle.png}
  \caption{Two-circle MDP}
  \label{fig:circle}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
%   \includegraphics[height=5.0cm,width=7cm]{figures/CircleMDP_prob.png}
    \includegraphics[height=3.0cm,width=.8\textwidth]{figures/CircleMDP_prob.png}
  \caption{The probability of transitioning from A to B}
  \label{fig:circle_result}
\end{subfigure}
\caption{The two-circle MDP}
\end{figure*}
%
The algorithms for this domain, GeoffPAC, ACE, VOMPS, and ACE-STORM, are implemented with a tabular version, where value function and density ratio function is computed via dynamic programming. The behavior policy $\mu$ follows a uniform distribution, and $\pi(A \rightarrow B)$, the probability from A to B under the target policy $\pi$ is reported in  Fig.~\ref{fig:circle_result}. 
As shown in Fig.~\ref{fig:circle_result}, VOMPS and GeoffPAC gradually choose to transition from A to B so that the agent would take the route with blue color and obtain a reward of $+10$. Compared with GeoffPAC, VOMPS converges faster.
Both ACE-STORM and ACE move from A to C, and ACE-STORM converges faster than ACE. Moving from A to C is an inferior solution since the agent will take the route with green color and fail to obtain a higher reward.
The difference between asymptotic solutions of GeoffPAC/VOMPS and ACE/ACE-STORM is due to the difference between the objective functions $J_{\hat \gamma}, J_\mu$, and the difference in the training process is due to the STORM component integrated into VOMPS and ACE-STORM.

\begin{figure*}[htb!]
\centering
\begin{subfigure}{.44\textwidth}
  \centering
  \includegraphics[height=3.5cm,width=1.\textwidth]{figures/cartpole_smooth_onpol.png}
  \caption{Comparison with on-policy methods}
  \label{fig:cartpole:onpol}
\end{subfigure}
\begin{subfigure}{.44\textwidth}
  \centering
  \includegraphics[height=3.5cm,width=1.\textwidth]{figures/cartpole_smooth_offpol.png}
  \caption{Comparison with off-policy methods}
  \label{fig:cartpole:offpol}
\end{subfigure}
\caption{Results on \texttt{CartPoleContinuous-v0}}
\end{figure*}

\subsection{Classic Control}
We use \texttt{CartPoleContinuous-v0} for CartPole domain, which has a continuous action space within the range of $[-1,1]$.
A near-optimal policy can reach a Monte-Carlo return at the level of $57$ within a fixed horizon of $200$ timesteps.
As shown in Fig.~\ref{fig:cartpole:onpol}, VOMPS and ACE-STORM learn the near-optimal policy with around $200$K samples, while SVRPG and SRVR-PG need more than $400$K samples with larger dynamic variances. As Fig.~\ref{fig:cartpole:offpol} shows, ACE, GeoffPAC, and DDPG do not perform well in this domain. Although TD3 seems to learn faster at the beginning, it reaches an inferior solution with a mean return around $50$ a higher variance than VOMPS and ACE-STORM.


\subsection{Mujoco Robot Simulation}
Experiments are also conducted on two benchmark domains provided by OpenAI Gym, including \texttt{Hopper-v2} and \texttt{HalfCheetah-v2}. 
As shown in Fig.~\ref{fig:hopper:onpol},~\ref{fig:hopper}, both GeoffPAC and VOMPS can achieve higher Monte Carlo returns than other methods and converge faster within $1$M samples on \texttt{Hopper-v2}. Compared with GeoffPAC, the learning curve of VOMPS is smoother and has a smaller variance. 
The results on \texttt{HalfCheetah-v2} are shown in Fig.~\ref{fig:halfcheetah:onpol},~\ref{fig:halfcheetah}. Fig.~\ref{fig:halfcheetah:onpol} indicates that VOMPS and ACE-STORM outperform SVRPG and SRVR-PG by a large margin, and Fig.~\ref{fig:halfcheetah} demonstrates that VOMPS and ACE-STORM achieve a similar performance of GeoffPAC/DDPG/TD3, with obviously smaller variances. We also observe that ACE does not perform well in general, and DDPG has a very large variance in these two domains.

In addition, a $20\%$ action noise is added to both the learning process and evaluation process in order to compare the noise resistance ability of different approaches (aka, the action is multiplied by a factor of $1\pm 0.2\chi$, where $\chi$ is drawn from a $[0,1]$-range uniform distribution). As shown in Fig.~\ref{fig:hopper:noise:onpol},~\ref{fig:hopper:noise:offpol},~\ref{fig:halfcheetah:noise:onpol},~\ref{fig:halfcheetah:noise:offpol}, compared with results under the original noise-free setting, VOMPS, ACE-STORM, SVRPG, and SRVR-PG tend to be insensitive to disturbances than other methods, which validates the effectiveness of the stochastic variance reduction component of these algorithms. In particular, VOMPS and ACE-STORM appear to be empirically the most noise-resistant in these two domains. 



\begin{footnotesize}
\begin{figure*}[htb!]
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hopper_onp.png}
  \caption{Hopper}
  \label{fig:hopper:onpol}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/halfcheetah_onpol.png}
    \caption{HalfCheetah}
    \label{fig:halfcheetah:onpol}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hop_20act_onpol.png}
  \caption{Hopper (action noise)}
  \label{fig:hopper:noise:onpol}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hc_20act_onpol.png}
  \caption{{\footnotesize HC (action noise)}}
  \label{fig:halfcheetah:noise:onpol}
\end{subfigure}
\caption{Comparison with on-policy PG methods (Mujoco), ``HC'' is short for HalfCheetah.}
\end{figure*}

\begin{figure*}[htb!]
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hopper_offp.png}
  \caption{Hopper}
  \label{fig:hopper}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/halfcheetah_offpol.png}
    \caption{HalfCheetah}
    \label{fig:halfcheetah}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hop_20act_offpol.png}
  \caption{Hopper (action noise)}
  \label{fig:hopper:noise:offpol}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width = 1\textwidth]{figures/hc_20act_offpol.png}
    \caption{{\footnotesize HC (action noise)}}
  \label{fig:halfcheetah:noise:offpol}
\end{subfigure}
\caption{Comparison with off-policy PG methods (Mujoco), ``HC'' is short for HalfCheetah.}
\end{figure*}
\end{footnotesize}
